Beyond a Single Human Demonstration: Learning from Scored Trajectory Alternatives for End-to-End Driving

Human driving logs record only one trajectory per scene, leaving other feasible driving choices without explicit trajectory targets or quality labels. This limits supervision for end-to-end planners that generate and refine multiple candidate trajectories. Meanwhile, conditioning refinement on a large vision-language model adds substantial online inference cost. We propose DriveSTA, which extends autoregressive proposal generation and proposal-conditioned residual flow refinement with scored trajectory alternatives. For each training scene, we generate alternatives offline through smooth deformations of the recorded trajectory and evaluate their simulated execution against logged traffic. Diverse, high-quality alternatives supervise distinct proposals and define residual targets for quality-guided denoising, while candidates spanning the full score range train a scorer to assess driving quality. A shared joint-embedding predictive architecture (JEPA), adapted through masked video-feature prediction, encodes observed frames once and provides temporal context for both refinement and scoring. On NAVSIM v1 Navtest, DriveSTA ranks first among the compared planners trained on NAVSIM data alone. With expanded training data, DriveSTA-Scale achieves state-of-the-art results among the compared methods on Navtest and closed-loop HUGSIM, while reducing mean planner forward-pass latency by 73% relative to ChainFlow-VLA in matched evaluations.

==> arxiv_spacing.tex <==
% Readable arXiv text spacing, scoped to the main article and supplement.
% The first-page card and bibliography retain their own typography.
\makeatletter
\newcommand{\arxivtextspacing}{%
  \linespread{1}\selectfont
  \raggedbottom
  \raggedcolumns
  \setlength{\parskip}{3pt}%
  \setlist[itemize,enumerate]{%
    leftmargin=*,topsep=6pt,partopsep=0pt,itemsep=0pt,parsep=3pt}%
  % Restore the section/subsection spacing provided by the CVPR style.
  \def\cvprsection{\@startsection{section}{1}{\z@}%
    {-10pt}{7pt}{\large\bf}}%
  \def\cvprsubsection{\@startsection{subsection}{2}{\z@}%
    {-8pt}{5pt}{\elvbf}}%
  % Run-in heads use the same fixed paragraph gap as ordinary prose.
  \renewcommand{\paragraph}{\@startsection{paragraph}{4}{\z@}%
    {0pt}{-1em}{\normalfont\normalsize\bfseries}}%
}
% Protect the two-column article from isolated paragraph lines.
\newcommand{\arxivmainflow}{%
  \clubpenalty=10000
  \widowpenalty=10000
  \displaywidowpenalty=10000
}
% Apply from the experimental tables onward, after the method's page layout.
\newcommand{\arxivfloatspacing}{%
  % Fixed, readable gaps between stacked floats and the surrounding text.
  \setlength{\floatsep}{10pt}%
  \setlength{\dblfloatsep}{10pt}%
  \setlength{\textfloatsep}{12pt}%
  \setlength{\dbltextfloatsep}{12pt}%
  \setlength{\intextsep}{12pt}%
}
\makeatother


==> sections/00_abstract.tex <==
% % Edited by Xinyao: 本文在考虑需要解决的两个问题，写作采取背景+问题：(1)一段驾驶场景仍旧存在很多高价值的监督目标(或驾驶策略)值得被挖掘；目前针对轨迹精炼使用VLM往往带来极高的时延代价需要被优化。
% Human driving logs record only one executed trajectory per scene, but the same scene can admit multiple reasonable driving choices. For end-to-end planners that generate and refine multiple candidates, these logs provide no explicit trajectory targets for unexecuted alternatives, while conditioning refinement on large vision-language models (VLMs) incurs substantial online inference latency.
%
% % Edited by Xinyao: 方法部分：为了解决上述问题，引出我们的方法并且简单介绍方法具体是什么，其次就是介绍方法里面每一点的设计优化+定性结果，形成逻辑框架。
% To address these limitations, we propose DriveSTA, an end-to-end planner that combines execution-validated trajectory supervision with efficient temporal conditioning from a shared JEPA encoder. Specifically, we construct multiple trajectory alternatives from the single demonstration in each scene, evaluate their execution, and retain diverse, high-quality targets for learning. These targets supervise trajectory generation and refinement, while execution scores teach the planner to assess candidate quality, helping it learn effective driving behaviors and make better choices. Furthermore, we replace online VLM conditioning with a JEPA encoder adapted through masked video-feature prediction, sharing a single encoding of observed frames across refinement and scoring. The resulting planner improves driving performance while reducing online inference latency.
%
% % Edited by Xinyao: 最后定量的展示结果，展示在四个基准上面的综合表现，以及在Navsim-Only和HUGSIM达到Rank #1的水平。
% Across four benchmark settings, DriveSTA variants achieve Rank #1 on Navtest under NAVSIM-only training with 95.1 PDMS and Rank #1 on HUGSIM with 56.1 RC and 46.7 HD-Score. They also achieve 91.3 EPDMS on Navtest and 56.1 EPDMS on Navhard.
%
Human driving logs record only one trajectory per scene, leaving other feasible driving choices without explicit trajectory targets or quality labels. This limits supervision for end-to-end planners that generate and refine multiple candidate trajectories. Meanwhile, conditioning refinement on a large vision-language model adds substantial online inference cost. We propose \method{}, which extends autoregressive proposal generation and proposal-conditioned residual flow refinement with scored trajectory alternatives. For each training scene, we generate alternatives offline through smooth deformations of the recorded trajectory and evaluate their simulated execution against logged traffic. Diverse, high-quality alternatives supervise distinct proposals and define residual targets for quality-guided denoising, while candidates spanning the full score range train a scorer to assess driving quality. A shared joint-embedding predictive architecture (JEPA), adapted through masked video-feature prediction, encodes observed frames once and provides temporal context for both refinement and scoring. On NAVSIM v1 Navtest, \method{} ranks first among the compared planners trained on NAVSIM data alone. With expanded training data, \method{}-Scale achieves state-of-the-art results among the compared methods on Navtest and closed-loop HUGSIM, while reducing mean planner forward-pass latency by 73\% relative to ChainFlow-VLA in matched evaluations.
\looseness=-1\relax\par


==> sections/00_arxiv_icons.tex <==
% Vector and brand icons, pre-rendered outside the card TikZ picture.
\newcommand{\arxivprojecticon}{%
  \tikz[x=1pt,y=1pt,baseline=0pt,draw=ArxivLink,line width=.55pt]{%
    \useasboundingbox (0,0) rectangle (10,9);
    \draw (5,4.5) circle[radius=4pt];
    \draw (5,4.5) ellipse[x radius=1.8pt,y radius=4pt];
    \draw (1,4.5) -- (9,4.5);
    \draw (1.5,2.7) -- (8.5,2.7);
    \draw (1.5,6.3) -- (8.5,6.3);
  }%
}
\newcommand{\arxivhficon}{%
  \tikz[x=1pt,y=1pt,baseline=0pt,line cap=round,line join=round]{%
    \useasboundingbox (0,0) rectangle (10,9);
    \fill[orange!58!yellow] (5,5.2) circle[radius=3.4pt];
    \draw[brown!65!black,line width=.5pt]
      (2.9,5.6) .. controls (3.5,6.4) .. (4.1,5.6)
      (5.9,5.6) .. controls (6.5,6.4) .. (7.1,5.6);
    \draw[brown!65!black,line width=.5pt]
      (3.7,4.6) .. controls (4.3,3.4) and (5.7,3.4) .. (6.3,4.6);
    \filldraw[fill=orange!58!yellow,draw=orange!70!brown,line width=.25pt]
      (4.3,1) .. controls (2,-.1) and (.2,1.7) .. (.5,3)
      -- (1,4.3) -- (1.9,2.9) -- (2,4.8) -- (2.8,3)
      -- (3.4,4.5) -- (3.8,2.8) -- (4.9,3.3) -- (5.1,2.5) -- cycle;
    \filldraw[fill=orange!58!yellow,draw=orange!70!brown,line width=.25pt]
      (5.7,1) .. controls (8,-.1) and (9.8,1.7) .. (9.5,3)
      -- (9,4.3) -- (8.1,2.9) -- (8,4.8) -- (7.2,3)
      -- (6.6,4.5) -- (6.2,2.8) -- (5.1,3.3) -- (4.9,2.5) -- cycle;
  }%
}

% Render before the card's TikZ picture: nested TikZ paths inside a node can
% inherit its path construction state. Saved boxes keep icon geometry isolated.
\newsavebox{\arxivmailbox}
\newsavebox{\arxivcodebox}
\newsavebox{\arxivprojectbox}
\newsavebox{\arxivhfbox}
\sbox{\arxivmailbox}{\includegraphics[width=10pt]{figures/branding/gmail.png}}
\sbox{\arxivcodebox}{\includegraphics[width=10pt]{figures/branding/github.pdf}}
\sbox{\arxivprojectbox}{\arxivprojecticon}
\sbox{\arxivhfbox}{\arxivhficon}
\newcommand{\arxiviconalign}[1]{\raisebox{\dimexpr.5ex-.5\height\relax}{\makebox[11pt][c]{#1}}}
\newcommand{\arxivmailicon}{\arxiviconalign{\usebox{\arxivmailbox}}}
\newcommand{\arxivcodeicon}{\arxiviconalign{\usebox{\arxivcodebox}}}
\renewcommand{\arxivprojecticon}{\arxiviconalign{\usebox{\arxivprojectbox}}}
\renewcommand{\arxivhficon}{\arxiviconalign{\usebox{\arxivhfbox}}}


==> sections/00_teaser.tex <==
% Non-floating title-block figure: full text width, original aspect ratio.
\noindent\begin{minipage}{\textwidth}
\centering
\captionsetup{type=figure,skip=3pt,position=bottom}
\includegraphics[width=\textwidth]{figures/new_teaser.pdf}\par
\caption{\textbf{DriveSTA at a glance.} Left compares supervision paradigms. Center shows scored endpoints, candidate paths, and JEPA attention with bird's-eye comparisons. Trajectory colors indicate PDMS intervals. Right compares DriveSTA-Scale S2 with selected baselines using truncated scales per metric. Full comparisons appear in the result tables.}
\label{fig:teaser}
\end{minipage}\par
% A terminal zero-height box retains the gap in LaTeX's title-box measurement.
\vspace{18pt}\null

